A Hierarchical Architecture for Human-Robot Cooperation Processes

In this paper we propose FlexHRC+, a hierarchical human-robot cooperation architecture designed to provide collaborative robots with an extended degree of autonomy when supporting human operators in high-variability shop-floor tasks. The architecture encompasses three levels, namely for perception, representation, and action. Building up on previous work, here we focus on (i) an in-the-loop decision making process for the operations of collaborative robots coping with the variability of actions carried out by human operators, and (ii) the representation level, integrating a hierarchical AND/OR graph whose online behaviour is formally specified using First Order Logic. The architecture is accompanied by experiments including collaborative furniture assembly and object positioning tasks.

==> figTableAssembly/allRobot.tex <==
\begin{figure*}[!t]
	%\vspace*{0.0cm}
\centering
\begin{subfigure}[b]{0.20\textwidth}
\includegraphics[width=\textwidth]{figTableAssembly/RobotAll/B1-11}
\caption{}
\label{fig:p2_1}
\end{subfigure}
~
\begin{subfigure}[b]{0.20\textwidth}
\includegraphics[width=\textwidth]{figTableAssembly/B1-12}
\caption{}
\label{fig:p2_2}
\end{subfigure}
~
\begin{subfigure}[b]{0.20\textwidth}
\includegraphics[width=\textwidth]{figTableAssembly/RobotAll/B1-13}
\caption{}
\label{fig:p2_3}
\end{subfigure}
~
\begin{subfigure}[b]{0.20\textwidth}
\includegraphics[width=\textwidth]{figTableAssembly/RobotAll/B1-21}
\caption{}
\label{fig:p2_4}
\end{subfigure}

\begin{subfigure}[b]{0.20\textwidth}
\includegraphics[width=\textwidth]{figTableAssembly/RobotAll/B1-22}
\caption{}
\label{fig:p2_1}
\end{subfigure}
~
\begin{subfigure}[b]{0.20\textwidth}
\includegraphics[width=\textwidth]{figTableAssembly/RobotAll/B1-23}
\caption{}
\label{fig:p2_2}
\end{subfigure}
~
\begin{subfigure}[b]{0.20\textwidth}
\includegraphics[width=\textwidth]{figTableAssembly/RobotAll/B1-31}
\caption{}
\label{fig:p2_3}
\end{subfigure}
~
\begin{subfigure}[b]{0.20\textwidth}
\includegraphics[width=\textwidth]{figTableAssembly/RobotAll/B1-32}
\caption{}
\label{fig:p2_4}
\end{subfigure}

\begin{subfigure}[b]{0.20\textwidth}
\includegraphics[width=\textwidth]{figTableAssembly/RobotAll/B1-33}
\caption{}
\label{fig:p2_1}
\end{subfigure}
~
\begin{subfigure}[b]{0.20\textwidth}
\includegraphics[width=\textwidth]{figTableAssembly/RobotAll/B1-41}
\caption{}
\label{fig:p2_2}
\end{subfigure}
~
\begin{subfigure}[b]{0.20\textwidth}
\includegraphics[width=\textwidth]{figTableAssembly/RobotAll/B1-42}
\caption{}
\label{fig:p2_3}
\end{subfigure}
~
\begin{subfigure}[b]{0.20\textwidth}
\includegraphics[width=\textwidth]{figTableAssembly/RobotAll/B1-43}
\caption{}
\label{fig:p2_4}
\end{subfigure}



\caption{The robot connects all the legs to the tabletop.}
\label{fig:monitoring}
\end{figure*}

==> figTableAssembly/monitoring.tex <==
\begin{figure*}[!t]
	%\vspace*{0.0cm}
\centering
\begin{subfigure}[b]{0.20\textwidth}
\includegraphics[width=\textwidth]{figTableAssembly/B2-11}
\caption{}
\label{fig:p2_1}
\end{subfigure}
~
\begin{subfigure}[b]{0.20\textwidth}
\includegraphics[width=\textwidth]{figTableAssembly/B2-12}
\caption{}
\label{fig:p2_2}
\end{subfigure}
~
\begin{subfigure}[b]{0.20\textwidth}
\includegraphics[width=\textwidth]{figTableAssembly/B2-13}
\caption{}
\label{fig:p2_3}
\end{subfigure}
~
\begin{subfigure}[b]{0.20\textwidth}
\includegraphics[width=\textwidth]{figTableAssembly/B2-21}
\caption{}
\label{fig:p2_4}
\end{subfigure}

\begin{subfigure}[b]{0.20\textwidth}
\includegraphics[width=\textwidth]{figTableAssembly/B2-22}
\caption{}
\label{fig:p2_1}
\end{subfigure}
~
\begin{subfigure}[b]{0.20\textwidth}
\includegraphics[width=\textwidth]{figTableAssembly/B2-23}
\caption{}
\label{fig:p2_2}
\end{subfigure}
~
\begin{subfigure}[b]{0.20\textwidth}
\includegraphics[width=\textwidth]{figTableAssembly/B2-31}
\caption{}
\label{fig:p2_3}
\end{subfigure}
~
\begin{subfigure}[b]{0.20\textwidth}
\includegraphics[width=\textwidth]{figTableAssembly/B2-32}
\caption{}
\label{fig:p2_4}
\end{subfigure}

\begin{subfigure}[b]{0.20\textwidth}
\includegraphics[width=\textwidth]{figTableAssembly/B2-33}
\caption{}
\label{fig:p2_1}
\end{subfigure}
~
\begin{subfigure}[b]{0.20\textwidth}
\includegraphics[width=\textwidth]{figTableAssembly/B2-41}
\caption{}
\label{fig:p2_2}
\end{subfigure}
~
\begin{subfigure}[b]{0.20\textwidth}
\includegraphics[width=\textwidth]{figTableAssembly/B2-42}
\caption{}
\label{fig:p2_3}
\end{subfigure}
~
\begin{subfigure}[b]{0.20\textwidth}
\includegraphics[width=\textwidth]{figTableAssembly/B2-43}
\caption{}
\label{fig:p2_4}
\end{subfigure}



\caption{The sequence of actions by the human to monitor the connections between the legs and the tabletop.}
\label{fig:monitoring}
\end{figure*}

==> figTableAssembly/tabletopPlacement.tex <==
\begin{figure}[!t]
	%\vspace*{0.0cm}
\centering
\begin{subfigure}[b]{0.4\columnwidth}
\includegraphics[width=\columnwidth]{figTableAssembly/A1}
\caption{}
\label{fig:p2_1}
\end{subfigure}
~
\begin{subfigure}[b]{0.4\columnwidth}
\includegraphics[width=\columnwidth]{figTableAssembly/A2}
\caption{}
\label{fig:p2_2}
\end{subfigure}

\begin{subfigure}[b]{0.4\columnwidth}
\includegraphics[width=\columnwidth]{figTableAssembly/A3}
\caption{}
\label{fig:p2_3}
\end{subfigure}
~
\begin{subfigure}[b]{0.4\columnwidth}
\includegraphics[width=\columnwidth]{figTableAssembly/A4}
\caption{}
\label{fig:p2_4}
\end{subfigure}

\begin{subfigure}[b]{0.4\columnwidth}
\includegraphics[width=\columnwidth]{figTableAssembly/A5}
\caption{}
\label{fig:p2_5}
\end{subfigure}
~
\begin{subfigure}[b]{0.4\columnwidth}
\includegraphics[width=\columnwidth]{figTableAssembly/A6}
\caption{}
\label{fig:p2_5}
\end{subfigure}

\caption{The sequence of actions associated with tabletop placement by the robot.}
\label{fig:tabletopPlacement}
\end{figure}
